Zooming Cautiously: Linear-Memory Heuristic Search With Node Expansion Guarantees

We introduce and analyze two parameter-free linear-memory tree search algorithms. Under mild assumptions we prove our algorithms are guaranteed to perform only a logarithmic factor more node expansions than A* when the search space is a tree. Previously, the best guarantee for a linear-memory algorithm under similar assumptions was achieved by IDA*, which in the worst case expands quadratically more nodes than in its last iteration. Empirical results support the theory and demonstrate the practicality and robustness of our algorithms. Furthermore, they are fast and easy to implement.

==> Linear-Memory Heuristic Search with Node Expansion Guarantees (1)/base.tex <==
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

\newcommand{\indicator}[1]{\llbracket #1 \rrbracket}

\definecolor{darkred}{rgb}{.7,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkblue}{rgb}{0,0,.8}
\definecolor{darkcyan}{rgb}{0,0.6,.6}
\definecolor{darkorange}{rgb}{.8,.4,0}
\definecolor{gray}{rgb}{.4,.4,.4}

\newcommand{\Nopt}{N_*}
\newcommand{\textred}[1]{\textcolor{darkred}{#1}}
\newcommand{\textblue}[1]{\textcolor{darkblue}{#1}}
\newcommand{\textcyan}[1]{\textcolor{darkcyan}{#1}}
\newcommand{\textgreen}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\textorange}[1]{\textcolor{darkorange}{#1}}
\newcommand{\redbf}[1]{\textcolor{darkred}{\textbf{#1}}}
\newcommand{\bluebf}[1]{\textcolor{darkblue}{\textbf{#1}}}
\newcommand{\greenbf}[1]{\textcolor{darkgreen}{\textbf{#1}}}
\newcommand{\orangebf}[1]{\textcolor{darkorange}{\textbf{#1}}}
\newcommand{\graybf}[1]{\textcolor{gray}{\textbf{#1}}}

%
\newcommand{\todo}[1]{\textcolor{darkorange}{(\emph{TODO: #1})}}
\newcommand{\comment}[1]{\textcolor{darkblue}{(\emph{#1})}}
\newcommand{\warning}[1]{\textcolor{red}{(\emph{WARNING: #1})}}
\newcommand{\quest}[1]{\textcolor{darkgreen}{(\emph{Q: #1})}}
\newcommand{\XXX}{\textcolor{red}{\textbf{XXX}}}

\newcommand{\Naturals}{\mathbb{N}_1}
\newcommand{\Nonnegints}{\mathbb{N}_0}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Rationals}{\mathbb{Q}}
%
\newcommand{\ie}{\emph{i.e.}, }
\newcommand{\eg}{\emph{e.g.}, }

\DeclareMathOperator*{\expect}{\mathbb{E}}
\DeclareMathOperator*{\argmax}{\text{argmax}}
\DeclareMathOperator*{\argmin}{\text{argmin}}

\newcommand{\D}{\text{d}}

\newcommand{\eps}{\varepsilon}
\newcommand{\half}{\tfrac{1}{2}}

\newcommand{\ceiling}[1]{\left\lceil#1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}


==> Linear-Memory Heuristic Search with Node Expansion Guarantees (1)/ubs.tex <==
\newcommand{\ubslong}{Uniform Budgeted Scheduler}
\newcommand{\ubs}{\text{UBS}}
\newcommand{\ceil}[1]{\lceil#1\rceil}

\section{Uniform Budgeted Scheduler}

\begin{figure}[bt!]
\begin{lstlisting}[label=lst:ubs,caption={The \ubslong. Programs could maintain an internal state and share a global state.}]
# T(k,n): cost of node (k, n) where program k runs for the n-th segment
def (*\ubs*)(T):
  q := make_priority_queue(T)
  insert(q, (1, 1))  # k=1, n=1
  while not empty(q):
    # Remove node of minimum T cost
    (k, n) := extract_min(q)
    res := run prog k for T(k, n) - T(k, n-1) steps
    if solution(res): return res
    # Push children onto the queue
    if not halted(res): insert(q, (k, n+1))
    if n == 1: insert(q, (k+1, 1))
  return None
\end{lstlisting}
\end{figure}

The \ubslong\ (\ubs) (see \cref{lst:ubs})
runs a growing and unbounded number of programs in dovetailing fashion.
At each iteration of the loop, the scheduler chooses a program $k$ to be run for
its $n$th segment.
This program may return with a solution in which case the scheduler does so too,
or it may halt in which case it will not appear in the queue anymore; otherwise, a new node $(k, n+1)$ is pushed onto the queue
as a request to run program $k$ for at least one more segment in a further iteration of the main loop.
If a program $k$ runs for its first segment, a request to run 
program $k+1$ for its first segment is also pushed onto the queue.
The scheduler always chooses the program in the queue with minimum cost/runtime $T(k,n)$.
After its $n$th segment, program $k$ has run for at most $T(k, n) - T(k, n-1)$ steps,
which means that it has run in total for at most $T(k, n) - T(k, 0)$ steps.
In the following, we always take $T(k, 0) := 0$.
$T(k, n)$ with $k\in\Naturals$ and $n\in\Nonnegints$ must be monotone increasing in $n$ for fixed $k$ and also in $k$ for $n=1$.



\ubs{} maintains amortized(?) uniform runtime between all programs.
This is because UBS is performing a Uniform Cost Search (UCS)~\cite{russell2009aima} on the tree
where the root is $(k=1, n=1)$ and each node $(k, n)$ has one child $(k, n+1)$
(unless the program halts)
and each node $(k, 1)$ has an additional child $(k+1, 1)$: \\
\begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c}
\\
$(k=1,n=1)$ & $\rightarrow$ & $(k=1,n=2)$ & $\rightarrow$ & $(k=1, n=3)$ & $\rightarrow$ & $\ldots$ \\
$\downarrow$ &&&&&& \\
$(k=2,n=1)$ & $\rightarrow$ & $(k=2,n=2)$ & $\rightarrow$ & $(k=2, n=3)$ & $\rightarrow$ & $\ldots$ \\
$\downarrow$ &&&&&& \\
$(k=3,n=1)$ & $\rightarrow$ & $(k=3,n=2)$ & $\rightarrow$ & $(k=3, n=3)$ & $\rightarrow$ & $\ldots$ \\
$\downarrow$ &&&&&& \\
$\ldots$ &&&&&& \\
\end{tabular}

Since in UCS the costs must increase along the paths, this explains the required properties of monotonicity of $T$.

Each program $k$ halts after $\tau_k\in\Nonnegints\cup\{\infty\}$ computation steps.

Define $T_{k, n}(j) := \max_{m\in\Nonnegints} \{T(j, m): T(j, m) \leq T(k, n)\}$,
which will be shown to be the maximum cost that has been extracted from the queue for program $j$
after $k$ returns from its $n$th segment.


\begin{theorem}\label{thm:ubs}
When program $k$ returns from its $n$th segment,
the total number of steps $T_\ubs(k, n)$ performed by all programs run by UBS
is bounded by
\begin{align*}
    T_\ubs(k, n) &\leq \sum_{j\in\Nonnegints} \min\{\tau_j, T_{k, n}(j)\}\,, 
\end{align*}
\end{theorem}
\begin{proof}
Since \ubs{} is a uniform cost search with the tree structure described above,
when the node $(k, n)$ is expanded (and program $k$ runs for its $n$th segment)
no node of strictly larger cost has been expanded, that is,
if node $j \neq k$ has run for $m$ segments 
then we must have $T(j, m) \leq T_{k, n}(j)$.
Since program $j$ also halts after no more than $\tau_j$ steps, the result follows.
\end{proof}

\cref{thm:ubs} can be simplified by considering the worst case where all programs $j\neq k$ have not halted before $k$ and multiplying $T(k, n)$ by the number of programs that have run for at least one segment.
\begin{corollary}\label{cor:uds}
When program $k$ terminates its $n$th segment,
\begin{align*}
    T_\ubs(k, n) &\leq T(k,n)\max\{j: T(j,1) \leq T(k, n)\}\,.
\end{align*}
\end{corollary}
\begin{proof}
From \cref{thm:ubs} and the definition of $T_{k, n}(.)$:
\begin{align*}
    T_\ubs(k, n) &\leq
    \sum_{j\in\Naturals} T_{k, n}(j) \\
    &\leq |\{j: T_{k, n}(j) > 0\}| T(k,n) \\
    &= T(k,n)\max\{j: T(j,1) \leq T(k, n)\}\,.\qedhere
\end{align*}
\end{proof}
For example, with $T(k,n):=n2^k$, we have that 
$T_\ubs(k, n) \leq \floor{k + \log_2(n)}n2^k$,
which is what a more specific scheduler using Luby's sequence~\cite{luby1993speedup} would guarantee.

\section{Z3/\ubs}

\newcommand{\threshexceed}{\thresh_\text{exceed}}

Define $\threshexceed(B) := \min \{\thresh :N(\thresh) \geq B \}$ be the first threshold for which the budget is exceeded.
Define $\thresh_k := \threshexceed(2^k)$. % COULD USE B_k here for a generic budget

Z3/\ubs{} uses \ubs{} where a program $k$
performs a budgeted exponential search where at each segment $BoundedSearch$ is called with a threshold and budget $2^k$.
This call will return with a solution if only if $\thresh \in [\thresh^*, \thresh_k)$,
which implies that the budget must be sufficient, that is, 
$ \thresh_k > \thresh^*$.
If $ \thresh_k \leq \thresh^*$, then program $k$ will never find a solution,
and over the sequence of segments the interval around $\thresh_k$ will continue to shrink forever, unless more information is available to prove that no solution can be found so as to halt the program.

Let $K := \ceil{\log_2 N_*}$ be the index of the first program $k$ for which $\thresh_k > \thresh^*$ (that is $2^K \geq N_*$)
and let $n$ be the number of segments it
for the exponential search to try a value in $[\thresh^*, \thresh_K)$
and return with a solution.
Then \cref{cor:uds} ensures that Z3/\ubs{} does not expand more than 
$\floor{K + \log_2(n)}n2^K
\leq 
2(\ceil{\log_2 N_*} + \floor{\log_2(n)})nN_*$
nodes before returning with a solution

Observe that this result holds even if programs $k < K$ do not halt.
\todo{generalize this to any $k \geq K$}


\todo{When we have information of when to halt the programs $k < K$, we can provide
another bound using \cref{thm:ubs} showing that Z3/UBS is within a $\log_2(n)\approx \log_2\log_2(\thresh^*/\fgapmin)$ factor of the iterative version that
monotonically increases the budget. }



==> Linear-Memory Heuristic Search with Node Expansion Guarantees (1)/zoomer_proof.tex <==


\begin{theorem}\label{thm:zoomer}
Assuming $\fcost$(root) > 0, \zoomer{} returns an optimal solution
after expanding no more nodes than
\begin{align*}
    \sum_{k=0}^\infty \nodecount_k \leq \max\left\{1, 4\zoomfact\right\}\nodecount^*\,,
\end{align*}
where $\zoomfact := \ceiling{\log_2(\thresh^*/\thresh_0)} + \ceiling{\log_2(\thresh^*/\fgapmin)}\,.$ 
\end{theorem}
\begin{proof}

Let $B_k := \nodecount_0 2^k$ be the expansion budget at iteration $k$ and 
define the minimum cost $\thresh_k$ at which the budget is exceeded:
$\thresh_k := \min_{\node\in\nodeset} \{\fcost(\node):\nodecount(\fcost(\node)) > B_k\}\,,$ 
and let $K := \min\{k\in\Nonnegints: B_k \geq \nodecount^*\} = \ceiling{\log_2(\nodecount^*/\nodecount_0)}$
be the first iteration with enough budget to find a solution.

Observe that \deepening{} with budget $B_k$ ensures that when it returns 
with \outabudget{} along with the return value $\threshdown$,
if we call again $\deepening(\text{root}, \threshdown, B_k)$ it will also return with \outabudget{},
which means that $\thresh_k \leq \threshdown$ and so we always have $\upper \geq \thresh_k$ (\cref{zoom:reduce_upper}).
Similarly, the algorithm also ensures that we always have $\llower < \thresh_k$.

\paragraph{Iterations $k< K$}
Now, suppose that at some point we have $\upper - \llower \leq \fgapmin$.
Then we have $\upper \leq \llower + \fgapmin < \thresh_k + \fgap(\thresh_k)$
which by \cref{zoom:reduce_upper} implies that $\upper = \thresh_k$.
We also have $\llower \geq \upper - \fgapmin = \thresh_k - \fgapmin$
which by \cref{zoom:set_up_min} implies that \texttt{up\_min} $= \thresh_k=\upper$, which means that no solution exists in $[\llower, \upper]$
since $\llower + \fgap(\llower)=\texttt{up\_min}=\upper$.
Therefore, iteration $k<K$ terminates no later than when $\upper - \llower \leq \fgapmin$ 
 (\cref{zoom:while}).
%Moreover, if $\upper \leq \texttt{up\_min}$ (\cref{zoom:while}) then $\llower +\fgap(\llower) = \texttt{up\_min} \geq \thresh_k$ 
%and thus no solution can be found at iteration $k$.
\iffalse
Furthermore, for iteration $K$
the algorithm must have returned with an optimal solution
\emph{before} having $\upper - \llower \leq \fgapmin$
since $\thresh_K > \llower \geq \thresh_K - \fgapmin $
would imply by \cref{zoom:increase_lower} that \deepening{}
was called with $\thresh\in [\thresh_K - \fgapmin, \thresh_K)$
which must return an optimal solution within budget.
\fi


For $a_k$ times the algorithm goes through \cref{zoom:double}
before calling \deepening,
and thus \llower{} is doubled until $\thresh=2 \times \llower \geq \thresh_k$
when \deepening{} returns with \outabudget,
at which point \upper{} is set to $\threshdown \leq \thresh$;
Together with 
$\llower < \thresh_k$ (by definition of $\thresh_k$),
this implies that $\upper - \llower \leq \thresh - \llower = \llower \leq \thresh_k$.
Thus, starting at worst from $\thresh_0$,
\begin{align*}
    a_k \leq \min\{d\in\Nonnegints:\thresh_0 2^d \geq \thresh_k \} 
    &= \ceiling{\log_2(\thresh_k/\thresh_0)} \\
    &\leq \ceiling{\log_2(\thresh^*/\thresh_0)} \,.
\end{align*}
Thereafter, for $b_k$ times
the algorithm goes through \cref{zoom:half}
before calling \deepening{} until  $\upper - \llower \leq \fgapmin$.
Hence
\begin{align*}
    b_k \leq \min\{d\in\Nonnegints:\thresh_k/2^d \leq \fgapmin\} &= \ceiling{\log_2(\thresh_k/\fgapmin)}  \\
    &\leq 
    \ceiling{\log_2(\thresh^*/\fgapmin)}\,.
\end{align*}


%% EDITOR NOTICE: Do keep \fgapopt because it is used for Z3's proof
\paragraph{Iteration $K$}
For iteration $K$ things are slightly different.
We still have $\llower < \thresh^*$
(otherwise a solution would have already been found)
and $\upper \geq \thresh_K$.
Assume that at some point $\upper - \llower \leq  2\fgapopt$.
Since $\upper$ is set, the algorithm goes through \cref{zoom:half}
before calling \deepening{}.
Thus $\thresh = (\upper+\llower)/2 \leq \llower + \fgapopt < \thresh^*+\fgapopt$
and similarly $\thresh \geq \upper - \fgapopt \geq \thresh_K - \fgapopt \geq \thresh^*$ where the last inequality is because there is enough budget for 
$\thresh^*$ by definition of $K$ but not for $\thresh_K$.
This implies that $\thresh \in [\thresh^*, \thresh^*+\fgap^*)$
and thus the call to \deepening{} returns with an optimal solution within budget.

Starting from the lower bound $\thresh_0$, the number of calls to \deepening{} 
after going through \cref{zoom:double}
before $\thresh \geq \thresh^*$ is less than $\ceiling{\log_2(\thresh^*/\thresh_0)}$.
At this point, either $\thresh \in [\thresh^*, \thresh_K)$
and an optimal solution is returned,
or $\thresh \geq \thresh_K$.
In the latter case, $\upper := \threshdown \leq \thresh = 2\llower$,
and since $\llower < \thresh^*$ we have $\upper - \llower < \thresh^*$.
Subsequently the number of calls to \deepening{}
after going through \cref{zoom:half} is at most
\begin{align*}
    \min\{d\in\Nonnegints:{} \thresh^*/2^d \leq 2\fgapopt\}
    %&\!=\! \ceilingpos{\log_2( (\upper_1-\llower_1) / (2\fgapopt) )} 
    &\leq\ceilingpos{\log_2( \thresh^* / (2\fgapopt) )}
    \\
    &\leq  \ceilingpos{\log_2( \thresh^* / \fgapmin )} \,.
\end{align*}

Therefore, over all iterations $k \leq K$ and including the first call to \deepening{},
when $\zoomfact \geq 1$
the number of node expansions is bounded by
\begin{equation*}
    \nodecount_0 + \sum_{k=1}^K (a_k + b_k) B_k 
    \leq \sum_{k=0}^K \zoomfact B_k
    \leq 2\zoomfact \nodecount_0 2^K 
    \leq 4\zoomfact \nodecount^*\,.
    \qedhere
\end{equation*}

\end{proof}

%%%%%%%% NECESSITY OF THETA- %%%%%%%%
\iffalse
Unfortunately, it is more than just an optimization. Without it the theorem wouldn't hold even approximately. Let me explain with a more concrete example.

Assume we set upper := $\thresh$ instead of upper := $\threshdown$.
Suppose that for some iteration k < K, the threshold $\thresh_k = 2^a+\eps$ for some $a$, and that f(root) = 1 = lower.
Initially you double lower until lower = $2^a$, and at this point  upmin = $2^a + \eps$, and upper = $2^{a+1}$.
Observe that there may be no node with value $2^a$, but there necessarily exists at least one node with value $\thresh_k$.
Now you need to halve the interval $[2^a, 2^{a+1}]$ until $\thresh$ falls into $[2^a, 2^a + \eps]$, which depends on ε which is *not* an f-gap and can be arbitrarily small, thus taking arbitrarily long to find out that there is no solution.

(The problem gets almost worse in the optimized version of Zoomer that doesn't double from the root at all k, but from a more arbitrary point.)

Setting upper := $\threshdown$ ensures that we only need $\thresh$ to fall into $[ 2^a, 2^a + \eps + \fgap(2^a + \eps) )$, which is an f-gap.

Initially, I thought of *lowering* lower to θ- before doubling, but then doubling wouldn't be doubling. To fix this, we could track (yet) another variable, one that truly doubles, and one that keeps lower. That would work, but then I thought of lowering upper instead, which works just as well.

\fi

==> Linear-Memory Heuristic Search with Node Expansion Guarantees (1)/zoomer_proof_tor.tex <==
\begin{theorem}\label{thm:zoomer}
Assuming $\theta_0 = \cost(\text{root}) > 0$,
\zoomer{} returns an optimal solution and the number of node expansions is at most
\begin{align*}
    \sum_{k=0}^{\infty} \nodecount_k \leq 4\zoomfact\nodecount^*\,,
\end{align*}
where
    $\zoomfact := \ceiling{\log_2 (\thresh^*/\thresh_0)} + \ceilingpos{\log_2 (\thresh^*/\precision)}$.
\end{theorem}

\begin{proof}
Let $B_k = N_0 2^k$ be the budget used in iteration $k$ and $k^* = \min\{k : B_k \geq N^*\}$. We complete the proof by showing two facts: 
\begin{enumerate}
\item[(1)] The algorithm never reaches iterations $k > k^*$. 
\item[(2)] The number of calls to \deepening{} in any iteration is at most $\omega$.
\end{enumerate}
Proof of (1): We prove the algorithm can never proceed from iteration $k^*$ to $k^*+1$. Notice that 
no iteration ends unless a solution has been found or \texttt{upper} is set. Subsequently, the definitions ensure that in iteration $k^*$,
\begin{align*}
N(\texttt{lower}) < N(\texttt{up\_min}) \leq  N(\theta^*) \leq B_{k^*} < N(\texttt{upper})\,.
\end{align*}
Hence it never occurs that $\texttt{up\_min} = \texttt{upper}$ and so the algorithm can only halt in iteration $k^*$ by finding the solution.

Proof of (2):
Suppose \zoomer{} starts iteration $k \leq k^*$. At the beginning of the iteration it doubles $\theta$ starting from some value at least as big as $\theta_0$ until either a solution is found or $N(\theta) > B_k$, which takes at most $\omega_1 = \lceil{\log_2(\theta^*/\theta_0)\rceil}$ calls to \deepening{}.
In subsequent periods where the algorithm chooses $\theta = (\texttt{upper} + \texttt{lower}) / 2$, the distance between \texttt{upper} and \texttt{lower} halves for the next period. Suppose instead that $\theta = \texttt{up\_min}$, which occurs when $(\texttt{upper} + \texttt{lower}) / 2 \leq \texttt{up\_min}$. In this case, one of three things happens:
    (a) A solution is found and the iteration ends.
    (b) The budget is exceeded, when \texttt{upper} is set to \texttt{up\_min} and the iteration ends.
    (c) The budget is not exceeded, \texttt{lower} is set to \texttt{up\_min} and the distance between \texttt{upper} and \texttt{lower} is halved.
In summary, after to each call to \deepening{} either the distance between \texttt{upper} and \texttt{lower} halves, or the iteration ends.
Therefore after at most 
$\omega_2 = \lceil\log_2(\theta^*/\fgapmin)\rceil$
additional calls to \deepening{} either the iteration has ended or $\texttt{upper} - \texttt{lower} \leq \fgapmin$. 
At this point, the definition of $\fgapmin$ means that $N(\theta) = N(\texttt{up\_min})$ and either the algorithm finds the solution if $k = k^*$ or $\texttt{upper} = \texttt{up\_min}$ in the following round for $k < k^*$.
Therefore the total number of calls to \deepening{} in iteration $k$ is at most $1 + \omega_1 + \omega_2$. 

Combining (1) and (2) shows that 
\begin{align*}
\sum_{k=0}^\infty N_k 
&\leq N_0(1 + \omega_1 + \omega_2)\sum_{k=0}^{k^*} 2^k 
\leq 4 \omega N^*\,, 
\end{align*}
where in the last inequality we used the geometric series to bound $\sum_{k=0}^{k^*} 2^k \leq 2^{k^* + 1}$ and the fact that $N_0 2^{k^*} \leq 2 N^*$.
\end{proof}


==> ubs.tex <==
\newcommand{\ubslong}{Uniform Budgeted Scheduler}
\newcommand{\ubs}{\text{UBS}}
\newcommand{\ceil}[1]{\lceil#1\rceil}

\section{Uniform Budgeted Scheduler}

\begin{figure}[bt!]
\begin{lstlisting}[label=lst:ubs,caption={The \ubslong. Programs could maintain an internal state and share a global state.}]
# T(k,n): cost of node (k, n) where program k runs for the n-th segment
def (*\ubs*)(T):
  q := make_priority_queue(T)
  insert(q, (1, 1))  # k=1, n=1
  while not empty(q):
    # Remove node of minimum T cost
    (k, n) := extract_min(q)
    res := run prog k for T(k, n) - T(k, n-1) steps
    if solution(res): return res
    # Push children onto the queue
    if not halted(res): insert(q, (k, n+1))
    if n == 1: insert(q, (k+1, 1))
  return None
\end{lstlisting}
\end{figure}

The \ubslong\ (\ubs) (see \cref{lst:ubs})
runs a growing and unbounded number of programs in dovetailing fashion.
At each iteration of the loop, the scheduler chooses a program $k$ to be run for
its $n$th segment.
This program may return with a solution in which case the scheduler does so too,
or it may halt in which case it will not appear in the queue anymore; otherwise, a new node $(k, n+1)$ is pushed onto the queue
as a request to run program $k$ for at least one more segment in a further iteration of the main loop.
If a program $k$ runs for its first segment, a request to run 
program $k+1$ for its first segment is also pushed onto the queue.
The scheduler always chooses the program in the queue with minimum cost/runtime $T(k,n)$.
After its $n$th segment, program $k$ has run for at most $T(k, n) - T(k, n-1)$ steps,
which means that it has run in total for at most $T(k, n) - T(k, 0)$ steps.
In the following, we always take $T(k, 0) := 0$.
$T(k, n)$ with $k\in\Naturals$ and $n\in\Nonnegints$ must be monotone increasing in $n$ for fixed $k$ and also in $k$ for $n=1$.



\ubs{} maintains amortized(?) uniform runtime between all programs.
This is because UBS is performing a Uniform Cost Search (UCS)~\cite{russell2009aima} on the tree
where the root is $(k=1, n=1)$ and each node $(k, n)$ has one child $(k, n+1)$
(unless the program halts)
and each node $(k, 1)$ has an additional child $(k+1, 1)$: \\
\begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c}
\\
$(k=1,n=1)$ & $\rightarrow$ & $(k=1,n=2)$ & $\rightarrow$ & $(k=1, n=3)$ & $\rightarrow$ & $\ldots$ \\
$\downarrow$ &&&&&& \\
$(k=2,n=1)$ & $\rightarrow$ & $(k=2,n=2)$ & $\rightarrow$ & $(k=2, n=3)$ & $\rightarrow$ & $\ldots$ \\
$\downarrow$ &&&&&& \\
$(k=3,n=1)$ & $\rightarrow$ & $(k=3,n=2)$ & $\rightarrow$ & $(k=3, n=3)$ & $\rightarrow$ & $\ldots$ \\
$\downarrow$ &&&&&& \\
$\ldots$ &&&&&& \\
\end{tabular}

Since in UCS the costs must increase along the paths, this explains the required properties of monotonicity of $T$.

Each program $k$ halts after $\tau_k\in\Nonnegints\cup\{\infty\}$ computation steps.

Define $T_{k, n}(j) := \max_{m\in\Nonnegints} \{T(j, m): T(j, m) \leq T(k, n)\}$,
which will be shown to be the maximum cost that has been extracted from the queue for program $j$
after $k$ returns from its $n$th segment.


\begin{theorem}\label{thm:ubs}
When program $k$ returns from its $n$th segment,
the total number of steps $T_\ubs(k, n)$ performed by all programs run by UBS
is bounded by
\begin{align*}
    T_\ubs(k, n) &\leq \sum_{j\in\Nonnegints} \min\{\tau_j, T_{k, n}(j)\}\,, 
\end{align*}
\end{theorem}
\begin{proof}
Since \ubs{} is a uniform cost search with the tree structure described above,
when the node $(k, n)$ is expanded (and program $k$ runs for its $n$th segment)
no node of strictly larger cost has been expanded, that is,
if node $j \neq k$ has run for $m$ segments 
then we must have $T(j, m) \leq T_{k, n}(j)$.
Since program $j$ also halts after no more than $\tau_j$ steps, the result follows.
\end{proof}

\cref{thm:ubs} can be simplified by considering the worst case where all programs $j\neq k$ have not halted before $k$ and multiplying $T(k, n)$ by the number of programs that have run for at least one segment.
\begin{corollary}\label{cor:uds}
When program $k$ terminates its $n$th segment,
\begin{align*}
    T_\ubs(k, n) &\leq T(k,n)\max\{j: T(j,1) \leq T(k, n)\}\,.
\end{align*}
\end{corollary}
\begin{proof}
From \cref{thm:ubs} and the definition of $T_{k, n}(.)$:
\begin{align*}
    T_\ubs(k, n) &\leq
    \sum_{j\in\Naturals} T_{k, n}(j) \\
    &\leq |\{j: T_{k, n}(j) > 0\}| T(k,n) \\
    &= T(k,n)\max\{j: T(j,1) \leq T(k, n)\}\,.\qedhere
\end{align*}
\end{proof}
For example, with $T(k,n):=n2^k$, we have that 
$T_\ubs(k, n) \leq \floor{k + \log_2(n)}n2^k$,
which is what a more specific scheduler using Luby's sequence~\cite{luby1993speedup} would guarantee.

\section{Z3/\ubs}

\newcommand{\threshexceed}{\thresh_\text{exceed}}

Define $\threshexceed(B) := \min \{\thresh :N(\thresh) \geq B \}$ be the first threshold for which the budget is exceeded.
Define $\thresh_k := \threshexceed(2^k)$. % COULD USE B_k here for a generic budget

Z3/\ubs{} uses \ubs{} where a program $k$
performs a budgeted exponential search where at each segment $BoundedSearch$ is called with a threshold and budget $2^k$.
This call will return with a solution if only if $\thresh \in [\thresh^*, \thresh_k)$,
which implies that the budget must be sufficient, that is, 
$ \thresh_k > \thresh^*$.
If $ \thresh_k \leq \thresh^*$, then program $k$ will never find a solution,
and over the sequence of segments the interval around $\thresh_k$ will continue to shrink forever, unless more information is available to prove that no solution can be found so as to halt the program.

Let $K := \ceil{\log_2 N_*}$ be the index of the first program $k$ for which $\thresh_k > \thresh^*$ (that is $2^K \geq N_*$)
and let $n$ be the number of segments it
for the exponential search to try a value in $[\thresh^*, \thresh_K)$
and return with a solution.
Then \cref{cor:uds} ensures that Z3/\ubs{} does not expand more than 
$\floor{K + \log_2(n)}n2^K
\leq 
2(\ceil{\log_2 N_*} + \floor{\log_2(n)})nN_*$
nodes before returning with a solution

Observe that this result holds even if programs $k < K$ do not halt.
\todo{generalize this to any $k \geq K$}


\todo{When we have information of when to halt the programs $k < K$, we can provide
another bound using \cref{thm:ubs} showing that Z3/UBS is within a $\log_2(n)\approx \log_2\log_2(\thresh^*/\fgapmin)$ factor of the iterative version that
monotonically increases the budget. }



==> zoomer_proof_tor.tex <==
\begin{theorem}\label{thm:zoomer}
Assuming $\theta_0 = \cost(\text{root}) > 0$,
\zoomer{} returns an optimal solution and the number of node expansions is at most
\begin{align*}
    \sum_{k=0}^{\infty} \nodecount_k \leq 4\zoomfact\nodecount^*\,,
\end{align*}
where
    $\zoomfact := \ceiling{\log_2 (\thresh^*/\thresh_0)} + \ceilingpos{\log_2 (\thresh^*/\precision)}$.
\end{theorem}

\begin{proof}
Let $B_k = N_0 2^k$ be the budget used in iteration $k$ and $k^* = \min\{k : B_k \geq N^*\}$. We complete the proof by showing two facts: 
\begin{enumerate}
\item[(1)] The algorithm never reaches iterations $k > k^*$. 
\item[(2)] The number of calls to \deepening{} in any iteration is at most $\omega$.
\end{enumerate}
Proof of (1): We prove the algorithm can never proceed from iteration $k^*$ to $k^*+1$. Notice that 
no iteration ends unless a solution has been found or \texttt{upper} is set. Subsequently, the definitions ensure that in iteration $k^*$,
\begin{align*}
N(\texttt{lower}) < N(\texttt{up\_min}) \leq  N(\theta^*) \leq B_{k^*} < N(\texttt{upper})\,.
\end{align*}
Hence it never occurs that $\texttt{up\_min} = \texttt{upper}$ and so the algorithm can only halt in iteration $k^*$ by finding the solution.

Proof of (2):
Suppose \zoomer{} starts iteration $k \leq k^*$. At the beginning of the iteration it doubles $\theta$ starting from some value at least as big as $\theta_0$ until either a solution is found or $N(\theta) > B_k$, which takes at most $\omega_1 = \lceil{\log_2(\theta^*/\theta_0)\rceil}$ calls to \deepening{}.
In subsequent periods where the algorithm chooses $\theta = (\texttt{upper} + \texttt{lower}) / 2$, the distance between \texttt{upper} and \texttt{lower} halves for the next period. Suppose instead that $\theta = \texttt{up\_min}$, which occurs when $(\texttt{upper} + \texttt{lower}) / 2 \leq \texttt{up\_min}$. In this case, one of three things happens:
    (a) A solution is found and the iteration ends.
    (b) The budget is exceeded, when \texttt{upper} is set to \texttt{up\_min} and the iteration ends.
    (c) The budget is not exceeded, \texttt{lower} is set to \texttt{up\_min} and the distance between \texttt{upper} and \texttt{lower} is halved.
In summary, after to each call to \deepening{} either the distance between \texttt{upper} and \texttt{lower} halves, or the iteration ends.
Therefore after at most 
$\omega_2 = \lceil\log_2(\theta^*/\fgapmin)\rceil$
additional calls to \deepening{} either the iteration has ended or $\texttt{upper} - \texttt{lower} \leq \fgapmin$. 
At this point, the definition of $\fgapmin$ means that $N(\theta) = N(\texttt{up\_min})$ and either the algorithm finds the solution if $k = k^*$ or $\texttt{upper} = \texttt{up\_min}$ in the following round for $k < k^*$.
Therefore the total number of calls to \deepening{} in iteration $k$ is at most $1 + \omega_1 + \omega_2$. 

Combining (1) and (2) shows that 
\begin{align*}
\sum_{k=0}^\infty N_k 
&\leq N_0(1 + \omega_1 + \omega_2)\sum_{k=0}^{k^*} 2^k 
\leq 4 \omega N^*\,, 
\end{align*}
where in the last inequality we used the geometric series to bound $\sum_{k=0}^{k^*} 2^k \leq 2^{k^* + 1}$ and the fact that $N_0 2^{k^*} \leq 2 N^*$.
\end{proof}

